Making a prototype of Seoul historical sites chatbot using Langchain

In this paper, we are going to share a draft of the development of a conversational agent created to disseminate information about historical sites located in the Seoul. The primary objective of the agent is to increase awareness among visitors who are not familiar with Seoul, about the presence and precise locations of valuable cultural heritage sites. It aims to promote a basic understanding of Korea's rich and diverse cultural history. The agent is thoughtfully designed for accessibility in English and utilizes data generously provided by the Seoul Metropolitan Government. Despite the limited data volume, it consistently delivers reliable and accurate responses, seamlessly aligning with the available information. We have meticulously detailed the methodologies employed in creating this agent and provided a comprehensive overview of its underlying structure within the paper. Additionally, we delve into potential improvements to enhance this initial version of the system, with a primary emphasis on expanding the available data through our prompting. In conclusion, we provide an in-depth discussion of our expectations regarding the future impact of this agent in promoting and facilitating the sharing of historical sites.

==> old.tex <==
Introduction
Our burgeoning interest in the convergence of culture and technology has inspired us to embark on a journey to develop a chatbot focused on the historical sites in Seoul, Korea. With a rich tapestry of archaeological remains, Seoul represents a rich ground for cultural exploration and provides cultural insights. With providing transport accessibility and convenience, Seoul represents Korea in various aspects.

However, we acknowledge the presence of intercultural communication challenges and potential biases in training data that extend beyond language and culture. While limitations do exist, commendable performance has been observed. Our primary goal is to bridge the gap between foreigners and the intricate nuances of Korean heritage by providing a concise and informative interface. Furthermore, we aim to assess the current status in specific sites.

In the ensuing sections of this paper, we will delineate the methodologies utilized in the construction of the chatbot, emphasizing our reliance on Streamlit, Langchain and OpenAI API. Streamlit has empowered us to create an interactive and user-friendly web app, while Langchain has been instrumental in developing the natural language processing functionalities, enabling smooth and coherent interactions.

Following the methodological discourse, we will delve into the development process of the chatbot, elaborating on how we fused technology and information to create a reliable tool for cultural dissemination. We will elaborate on how we sourced and integrated data from an open API, orchestrated the logical flow, and optimized the user interface to ensure a seamless user experience.

Subsequently, we will discuss the advantages of deploying this chatbot, highlighting how it serves as a beacon for cultural enlightenment and facilitates intuitive learning for foreigners curious about Korean heritage. Despite its merits, we will also address the inherent limitations stemming from the restricted amount of data available through the open API and the focused scope of the chatbot on heritage sites in Seoul.

Finally, the paper will conclude with reflections on the implications of our work, examining how the chatbot stands as a testament to the potential of technology in fostering intercultural understanding and appreciation. We will contemplate the avenues for future enhancements and expansions, envisioning a broader and deeper scope encompassing diverse aspects of cultural heritage and interaction.

Through this paper, we aspire to shed light on the intricate process of developing a culturally enriched chatbot and spark discussions on leveraging technology for more inclusive and comprehensive cultural explorations.

-------------------------------------------------------------

-------------------------------------------------------------


Discussion
original contents
Exploring the intricacies of our heritage-focused chatbot reveals a spectrum of advantages and inherent limitations, forming a complex narrative of innovation, accessibility, and the need for refinement. On one hand, the chatbot emerges as a beacon of cultural knowledge, illuminating the rich tapestry of Seoul’s heritage to a global audience. It acts as a conduit, enabling foreigners to transcend language barriers and immerse themselves in the fascinating world of Korean heritage, thereby fostering a deeper appreciation and understanding of a culture that is rich and diverse.

This enlightening experience is heightened by the incorporation of state-of-the-art technologies such as Streamlit and Langchain, which ensure the user interface is not just visually appealing but also intuitively designed, enabling seamless interactions. The technological prowess of our chatbot allows for advanced natural language processing, facilitating meaningful and coherent conversations and providing users with a rich, educative experience that kindles interest and curiosity in Korean culture.

However, intertwined with these benefits are the limitations stemming from our reliance on open data, which act as the chatbot's lifeline, feeding it with the necessary information. This reliance renders the chatbot susceptible to the constraints of the available data, potentially leading to a lack of depth and breadth in the information provided. The limited scope of the open data could result in the omission of valuable heritage sites and detailed insightful descriptions, restricting the chatbot’s potential as a comprehensive cultural guide.

Compounding this is the imperative need for meticulous verification of the chatbot’s responses. Despite striving for accuracy and reliability, the complex nature of natural language processing and limitations in the existing data may introduce inaccuracies or generalized responses. This emphasizes the necessity for users to approach the provided information with caution, meticulously cross-verifying to ensure its reliability and accuracy when detailed and precise information is required.

Thus, the narrative of our chatbot is a woven tapestry of innovation, accessibility, and limitations, each thread contributing to its overall essence. While the chatbot stands as a pioneering tool in cultural education, sparking global interest and appreciation for Korean heritage, its inherent limitations underscore the importance of continuous enhancement and refinement. Navigating these limitations is vital to fully unlock the chatbot’s potential in bridging cultural divides and enriching the global cultural milieu, ensuring a more nuanced, accurate, and comprehensive portrayal of Seoul’s illustrious heritage. 
There are troubles when user tries to converse more about the historical sites in each location, because our data only contains the location and the name of the heritage. To derive more natural conversation from a little information, we prompted like “make conversation with the dataset”. In this prompt, the dataset means the json file where each line includes “main\_key”, “h\_eng\_dong”, “ h\_eng\_gu”, “name\_eng”, ”h\_eng\_city”. The result is like below.

<image or table section>

Referring to the result, we can help the users hardly resolving which prompt to use for obtaining more conversation and information. For example, after the user begins with the prompt asking about the heritages in specific location in seoul and chatbot immediately answers, we can show the multiple choice for appropriate prompts to continue the conversation. However, it can be possible that conversation ends and the user is not satisified. To solve this, we prompted like “show more preduct the questions of users when chatting about heritage in seoul”. The result is like below
With those possible questions related to our dataset, we can help users worrying about what to say when it is the first time to meet the chatbot or when the conversation has just ended. Furthermore, we can use the results for fine-tuning other Large Language Models. (self instruct) For example, when using the conversation, the LLM models can learn what questions they will get, and how to answer them. It is also beneficial when saving money as OpenAI charges a fee when using gpt3.5 or gpt4.

\begin{figure}[!ht]
\begin{center}
\includegraphics[scale=0.3]{answer1.JPG} 
\caption{Conversation made by the prompt "make conversation with the dataset" -1}
\label{fig.3}
\end{center}
\end{figure}

\begin{figure}[!ht]
\begin{center}
\includegraphics[scale=0.4]{answer2.JPG} 
\caption{Conversation made by the prompt "make conversation with the dataset" -2}
\label{fig.4}
\end{center}
\end{figure}

\begin{figure}[!ht]
\begin{center}
\includegraphics[scale=0.4]{answer3.png} 
\caption{Our chatbot response for the prompt "suggest further questions on Seoul's heritage." -1}
\label{fig.5}
\end{center}
\end{figure}

\begin{figure}[!ht]
\begin{center}
\includegraphics[scale=0.4]{answer4.png} 
\caption{Our chatbot Response for the prompt "suggest further questions on Seoul's heritage." -2}
\label{fig.6}
\end{center}
\end{figure}
